Doc2Spec: Synthesizing Formal Programming Specifications from Natural Language via Grammar Induction

Ensuring that API implementations and usage comply with natural language programming rules is critical for software correctness, security, and reliability. Formal verification can provide strong guarantees but requires precise specifications, which are difficult and costly to write manually. To address this challenge, we present Doc2Spec, a multi-agent framework that automatically induces a domain-specific grammar from natural-language API rules and uses it to guide specification generation. Doc2Spec fixes a domain-agnostic logical skeleton as a grammar template, prompts LLMs to infer domain-specific predicates and sorts, and formalizes each rule within the resulting grammar, turning an unreliable one-shot translation into a sequence of constrained, checkable steps. Across six benchmarks spanning Solidity and Rust, Doc2Spec improves precision by 0.28 and recall by 0.37 over baselines that lack grammar induction or perform it in one unstaged step, demonstrating the benefits of grammar-guided formalization and the staged pipeline. Moreover, its formalized rules enable symbolic-execution tools to uncover 142 previously unknown rule violations, confirming the rules' correctness and practical usefulness.

==> appendices/prompt_artifacts/01_entity_scope_discovery.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseField{Entity patterns}{None (empty list).}
\ResponseField{Scope patterns}{None (empty list).}


==> appendices/prompt_artifacts/02_entity_entity_discovery.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseGroup{Entity patterns: 1}
\ResponseField{Kind}{\texttt{function}}
\ResponseField{Start regex}{\texttt{\textasciicircum{}function\textbackslash{}s+[A-Za-z\_][A-Za-z0-9\_]*\textbackslash{}b}}
\ResponseField{Example}{\texttt{function transferFrom(address \_from, address \_to, uint256 \_value) public returns (bool success)}}
\ResponseField{Scope patterns}{None (empty list).}


==> appendices/prompt_artifacts/03_entity_pattern_validation.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseGroup{entity-pattern-0001}
\ResponseField{Keep pattern}{\texttt{true}}
\ResponseField{Rationale}{Matches a Solidity function declaration, which is a valid entity definition for attaching behavioral documentation.}


==> appendices/prompt_artifacts/04_entity_candidate_classification.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseGroup{candidate-0001}
\ResponseField{Entity}{\texttt{true}}
\ResponseField{Declaration end line}{7}
\ResponseField{Enclosing scopes}{None (empty list).}
\ResponseField{Kind}{\texttt{function}}
\ResponseField{Name}{\texttt{transferFrom}}
\ResponseField{Visibility}{\texttt{public}}
\ResponseGroup{Parameters (declaration order)}
\begin{tabularx}{\linewidth}{@{}lXX@{}}
\toprule
\textbf{Position} & \textbf{Name} & \textbf{Type} \\
\midrule
1 & \texttt{\_from} & \texttt{address} \\
2 & \texttt{\_to} & \texttt{address} \\
3 & \texttt{\_value} & \texttt{uint256} \\
\bottomrule
\end{tabularx}\par
\ResponseGroup{Return values (declaration order)}
\begin{tabularx}{\linewidth}{@{}lXX@{}}
\toprule
\textbf{Position} & \textbf{Name} & \textbf{Type} \\
\midrule
1 & \texttt{success} & \texttt{bool} \\
\bottomrule
\end{tabularx}\par


==> appendices/prompt_artifacts/05_rule_clause_extraction.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseGroup{Clause 1}
Transfers \_value amount of tokens from address \_from to address \_to, and MUST fire the Transfer event.\par
\ResponseGroup{Clause 2}
Transfers of 0 values MUST be treated as normal transfers and fire the Transfer event.\par
\ResponseGroup{Clause 3}
The function SHOULD throw unless the \_from account has deliberately authorized the sender of the message via some mechanism.\par


==> appendices/prompt_artifacts/06_rule_candidate_scoring.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\begin{tabularx}{\linewidth}{@{}Xll@{}}
\toprule
\textbf{Candidate} & \textbf{Rule label} & \textbf{Confidence} \\
\midrule
\texttt{candidate-0003} & \texttt{true} & 0.8 \\
\bottomrule
\end{tabularx}\par
\ResponseGroup{candidate-0003: rationale}
Specifies a behavioral expectation (the function should throw when unauthorized), which can be tested; although not a MUST, it is still a non-vague, enforceable rule.\par


==> appendices/prompt_artifacts/07_predicate_semantic_analysis.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseGroup{C\_authorized}
\ResponseField{Role}{condition}
\ResponseField{Source span}{the \_from account has deliberately authorized the sender of the message via some mechanism}
\ResponseField{Meaning}{The \_from account has deliberately authorized the message sender via some mechanism}
\ResponseField{Parameters (in order)}{\texttt{\_from}, \texttt{sender}}
\ResponseGroup{O\_throw}
\ResponseField{Role}{obligation}
\ResponseField{Source span}{throw}
\ResponseField{Meaning}{The function reverts execution}
\ResponseField{Parameters (in order)}{None (empty list).}
\ResponseGroup{Boolean structure}
\ResponseField{Outcome formula}{\texttt{O\_throw}}
\ResponseField{Condition formula}{\texttt{not C\_authorized}}


==> appendices/prompt_artifacts/08_predicate_vocabulary_synthesis.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseGroup{Sorts}
\ResponseField{Address}{Ethereum address}
\ResponseGroup{Predicate: AuthorizedCondition}
\ResponseField{Source atom}{\texttt{C\_authorized}}
\ResponseField{Signature}{\texttt{AuthorizedCondition(\_from: Address, sender: Address)}}
\ResponseField{Meaning}{The \_from account has deliberately authorized the message sender via some mechanism}
\ResponseGroup{Predicate: ThrowObligation}
\ResponseField{Source atom}{\texttt{O\_throw}}
\ResponseField{Signature}{\texttt{ThrowObligation()}}
\ResponseField{Meaning}{The function reverts execution}


==> appendices/prompt_artifacts/09_formalize_dsl_translation.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseField{DSL statement}{\texttt{SHOULD ThrowObligation() if not AuthorizedCondition(\_from, sender);}}


==> appendices/prompt_artifacts/erc721_scope.response.tex <==
% Generated by scripts/render_response_views.py; edit the renderer, not this file.
\ResponseGroup{Scope patterns: 1}
\ResponseField{Kind}{\texttt{interface}}
\ResponseField{Start regex}{\texttt{\textasciicircum{}interface\textbackslash{}s+(?P<name>\textbackslash{}w+)\textbackslash{}b.*\textbackslash{}\{}}
\ResponseField{Example}{\texttt{interface ERC721Metadata /* is ERC721 */ \{}}
\ResponseField{Opening regex}{\texttt{\textbackslash{}\{}}
\ResponseField{Closing regex}{\texttt{\textbackslash{}\}}}
\ResponseField{Role}{\texttt{semantic\_container}}


==> appendices/prompt_tmpl/resolve_ebnf_error.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.
Available Actions:
- write_dsl: Return exactly one DSL statement that conforms to the provided grammar for the given rule.
  Input Schema: {
  "type": "object",
  "properties": {
    "dsl": {
      "type": "string",
      "description": "A single DSL statement that ends with ';' and parses with the grammar."
    }
  },
  "required": [
    "dsl"
  ]
}


Write ONE DSL statement for the given natural-language rule, using the following Lark grammar.
Rules:
- The DSL must parse with this grammar.
- Do NOT invent predicate names or change arity; only use what appears in the grammar.
- Output exactly one statement and end it with ';'.
- If rule requires certain attributes from the target(provided in JSON format), use JSON path to access them.

Grammar:```
(*@\hlline{0.11}@*){{grammar}}
```

Natural-language rule:```
(*@\hlline{0.11}@*){{sentence}}
```


Associated Target:```
(*@\hlline{0.10}@*){{entity}}
```

Target Attributes in JSON format:```
(*@\hlline{0.20}@*){{entity_attributes}}
```

Previous attempt and error (fix it): (*@\hlline{0.16}@*){{dsl}} {{error}}

Analyze the request step by step, then respond with JSON in the following format
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}
\end{lstlisting}
\end{llmex}

==> appendices/prompt_tmpl/resolve_json_error.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
Last Response:```
(*@\hlline{0.20}@*){{previous_response}}
```
There was an error processing the last response:```
(*@\hlline{0.09}@*){{error}}
``` 
Please refine your last response to fix the error.
Respond with JSON only, without any additional text.
\end{lstlisting}
\end{llmex}

==> appendices/prompt_tmpl/resolve_regex_error.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
Regex Pattern:```
(*@\hlline{0.11}@*){{pattern}}
```
Example to be matched:```
(*@\hlline{0.11}@*){{example}}
```
Error Message:```
(*@\hlline{0.09}@*){{error}}
```
Please provide a corrected regex pattern that resolves the error.
\end{lstlisting}
\end{llmex}

==> appendices/prompt_tmpl/resolve_schema_err.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
Data:```
(*@\hlline{0.26}@*){{previous_responsed_json}}
```
Schema:```
(*@\hlline{0.19}@*){{expected_schema}}
```
There was an error validating the data against the schema:```
(*@\hlline{0.09}@*){{error}}
```
Please refine the data to conform to the schema.
Respond with JSON only, without any additional text.
\end{lstlisting}
\end{llmex}

==> figure/1_entity_extractor.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.

Available Actions:

- new_target_patterns: New missing target patterns based on the chunk.
  Input Schema: {
  "type": "array",
  "items": {
    "type": "object",
    "properties": {
      "example": {
        "type": "string",
        "description": "An example line that matches the target pattern."
      },
      "pattern": {
        "type": "string",
        "description": "regex pattern to identify targets. For example, to identify function declarations, the pattern can be '^function\s+\w+\s*\(.*\)'."
      }
    },
    "required": [
      "pattern",
      "example"
    ]
  }
}

- new_exclude_patterns: New missing exclude regex patterns based on the chunk.
  Input Schema: {
  "type": "array",
  "items": {
    "type": "object",
    "properties": {
      "example": {
        "type": "string",
        "description": "An example line that matches the exclude pattern."
      },
      "pattern": {
        "type": "string",
        "description": "regex pattern to exclude certain lines from been considered as target. For example, to exclude lines that are comments."
      }
    },
    "required": [
      "pattern",
      "example"
    ]
  }
}


Chunk:```
(*@\hlline{0.09}@*){{chunk}}
```

Previous analyzed target patterns: (*@\hlline{0.27}@*){{previous_target_patterns}}

Exclude lines that match any of the following regex patterns from been considered as target: (*@\hlline{0.28}@*){{previous_exclude_patterns}}

Only call update_target_patterns if previous patterns is not enough to cover the target kinds in the current chunk.

Only call update_exclude_patterns if there are new patterns to exclude lines from been considered as target in the current chunk.

If current chunk does not contain any new target/exclude pattern, do not call update.

Example:

Chunk:```

<comment or description...>

function name() public view returns (string)

```

Previous analyzed target patterns: []

Return only new target regex patterns: ["^function\\s+\\w+\\s*\\(.*\\)"]

------

Chunk:```

<comment or description...>

event XXX

```

Previous analyzed target patterns: ["^function\s+\w+\s*\(.*\)"]

Return only new target regex patterns: ["^event\s+\w+\s*\(.*\)"]

```

Analyze the request step by step, then respond with JSON in the following format

{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}



\end{lstlisting}
\end{llmex}


==> figure/2_attribute_extractor_accumulation.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.
Available Actions:

- record_additional_attributes: Record any additional attributes of the target that are not already listed.
  Input Schema: {
  "type": "object",
  "properties": {
    "attributes": {
      "type": "array",
      "items": {
        "type": "object",
        "properties": {
          "name": {
            "type": "string",
            "description": "Name of the attribute."
          },
          "description": {
            "type": "string",
            "description": "Description of the attribute."
          },
          "schema": {
            "type": "object",
            "description": "JSON schema of the attribute value."
          }
        },
        "required": [
          "name",
          "description",
          "schema"
        ]
      }
    }
  },
  "required": [
    "attributes"
  ]
}



You are identifying attributes that can be extracted from a target.


Target: ```
(*@\hlline{0.1}@*){{entity}}
```


Existing attributes (JSON):```
(*@\hlline{0.25}@*){{accumulated_attributes}}
```

Identify additional attributes that are useful and present in this target.
Only include attributes that can be extracted from the target text.
Do not repeat existing attribute names.

Example:```
Target:
function add(a: int, b: int) -> int:

Attributes: {
  "name": "add",
  "parameters": [
    {"name": "a", "type": "int"},
    {"name": "b", "type": "int"}
  ],
  "return_type": "int"
}
```

Analyze the request step by step, then respond with JSON in the following format
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}

\end{lstlisting}
\end{llmex}

==> figure/2_attribute_extractor_extract.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.
Available Actions:
- record_attribute_values: Record extracted attribute values as a name -> value mapping.
  Input Schema: {
  "type": "object",
  "properties": {
    "attribute_values": {
      "type": "object",
      "description": "Mapping of attribute names to extracted values."
    }
  },
  "required": [
    "attribute_values"
  ]
}

Extract attribute values from the target.


Target:```
(*@\hlline{0.1}@*){{entity}}
```



Attributes to extract (JSON definitions):```
(*@\hlline{0.25}@*){{accumulated_attributes}}
```

Return only values that are explicitly supported by the target text.
If an attribute is not present, omit it.
Analyze the request step by step, then respond with JSON in the following format
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}
\end{lstlisting}
\end{llmex}

==> figure/3_rule_extractor_1boundary.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.
Available Actions:
- retry: More lines are needed to find the boundary line of description/comment.
  Input Schema: None
  
- found_boundary: Indicates that the upper boundary line of description/comment for the given target has been found.
  Input Schema:    {
  "type": "object",
  "properties": {
    "line": {
      "type": "integer",
      "description": "The line number where the upper boundary line is found."
    }
  },
  "required": [
    "line"
  ]
}




Determine the upper boundary of description/comment for the target "(*@\hlline{0.1}@*){{entity}}" in the given chunk.

- Upper boundary is the first line of the description/comment block that describes the target.

- Lower boundary is the last line of the description/comment block that describes the target.

- Do NOT include comments that belong to the previous/next target.

This is the chunk for description/comment of the target: ```
(*@\hlline{0.1}@*){{chunk}}
```

Example:```
Target at lines 63-64
Chunk:```

58    ...
59 }
60
61 // This function does Y.
62 // additional comment
63 void doY(
64    int param1,) {
65 ...
...
70 }
71
72 string helper() {
73    ...
```

Upper bound for upward context of target at lines 63-64 is at line 61 since upper is belong to the previous target.
Lower bound for downward context of target at lines 63-64 is at line 70 since next is belong to the next target.

```


Analyze the request step by step, then respond with JSON in the following format
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}
\end{lstlisting}
\end{llmex}

==> figure/3_rule_extractor_2sentence.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.
Available Actions:
- extract_sentence: Extracted all sentences that are relevant to the target within the given chunk.
  Input Schema: {
  "type": "array",
  "description": "List of extracted sentences. Each array item is a sentence string.",
  "items": {
    "type": "object",
    "properties": {
      "sentence": {
        "type": "string",
        "description": "A sentence that is relevant to the target."
      },
      "complete": {
        "type": "boolean",
        "description": "Whether the sentence is complete or not. If false, it means the sentence is incomplete and more lines are needed to complete it."
      }
    }
  }
}





Extract all sentences that are relevant to the given target "(*@\hlline{0.1}@*){{entity}}" within the chunk below.

```
(*@\hlline{0.1}@*){{chunk}}
```

The sentences should be exactly same as in the chunk.


Analyze the request step by step, then respond with JSON in the following format
\begin{lstlisting}[language=appendixjson]
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}
\end{lstlisting}
\end{llmex}

==> figure/3_rule_extractor_3score.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
Available Actions:
- judge_sentence: Judge whether the sentence is a normative rule that applies to the target.
  Input Schema: {
  "type": "object",
  "properties": {
    "reason": {
      "type": "string",
      "description": "The reason why the sentence is a normative rule or not."
    },
    "confidence": {
      "type": "number",
      "description": "The confidence score (between 0 and 1) that the sentence is a normative rule that applies to the target."
    },
    "is_rule": {
      "type": "boolean",
      "description": "Whether the sentence is a normative rule that applies to the target."
    }
  },
  "required": [
    "is_rule",
    "reason",
    "confidence"
  ]
}


Judge whether the following sentence is a normative rule that applies to the target "(*@\hlline{0.1}@*){{entity}}".

A normative rule is any statement that defines binding behavior, constraints, or guarantees for the given Target-i.e., something that must be true for a compliant implementation/usage, and is in principle testable (violations are meaningful).
A sentence is a rule if it specifies any of the following about the Target (even without modal verbs):

Obligations / prohibitions / permissions
Explicit: must, shall, should, may, may not, required to, prohibited, allowed to.
Conditional behavior (implicit normativity in descriptive mood)
Treat descriptive spec language as normative when it constrains correct behavior, e.g.
"returns X when/if ..." (postconditions)
"throws/raises/signals E if/when ..." (exception/error conditions)
"emits event when/if ..." (side effects / signaling)
"is set to / remains / equals / is undefined unless ..." (state/value constraints)
"only if / only when / if and only if / unless / otherwise ..." (necessary/sufficient conditions)

Invariants and quantifiable constraints
always, never, cannot, at least, at most, exactly, no more than, within N units, before/after.

Structured documentation tags / annotations that encode contract semantics
Content under tags like @param, @return, @throws/@exception, @pre, @post, @invariant, etc. should be treated as contract clauses when they impose conditions, guarantees, or failure modes.


Sentence: "(*@\hlline{0.12}@*){{sentence}}"


Analyze the request step by step, then respond with JSON in the following format
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}
\end{lstlisting}
\end{llmex}


==> figure/4_grammar_inferer_1sort.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.
Available Actions:
- add_sorts: Add sorts needed to formalize the rule.
  Input Schema: 
{
  "type": "array",
  "items": {
    "type": "object",
    "properties": {
      "name": {
        "type": "string",
        "description": "Name of the sort."
      },
      "description": {
        "type": "string",
        "description": "Description of the sort."
      }
    },
    "required": [
      "name",
      "description"
    ]
  }
}




You are a formalization assistant. Identify any missing sorts other than the existing ones needed to formalize the rule for the target.

Sentence:```
(*@\hlline{0.12}@*){{sentence}}
```

The sentence is in the context of the following

Target:```
(*@\hlline{0.1}@*){{entity}}
```

Existing sorts:```
(*@\hlline{0.20}@*){{accumulated_sorts}}
```

Example:```

Sentence: Socrates is human.

Sorts:

- Person: An individual human being.

```



Analyze the request step by step, then respond with JSON in the following format
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}
\end{lstlisting}
\end{llmex}

==> figure/4_grammar_inferer_2predicate.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.
Available Actions:
- add_predicates: Add predicates needed to formalize the rule.
  Input Schema: {
  "type": "array",
  "items": {
    "type": "object",
    "properties": {
      "name": {
        "type": "string",
        "description": "Name of the predicate."
      },
      "description": {
        "type": "string",
        "description": "Description of the predicate."
      },
      "primary": {
        "type": "boolean",
        "description": "Indicates if the predicate is primary."
      },
      "parameters": {
        "type": "object",
        "description": "Parameters of the predicate with their sorts. key is parameter name, value is sort name."
      }
    },
    "required": [
      "name",
      "description",
      "parameters"
    ]
  }
}




You are a formalization assistant. Identify any missing predicates other than the existing ones needed to formalize the rule for the target.
Primary predicate is the main predicate that define the core logic of this sentence, while normal predicates provide additional context, conditions or details.
Each sentence must have only one primary predicate. Zero or multiple other normal predicates are allowed.

Sentence:```
(*@\hlline{0.12}@*){{sentence}}
```

The sentence is in the context of the following

Target:```
(*@\hlline{0.1}@*){{target}}
```

Existing sorts:```
(*@\hlline{0.2}@*){{accumulated_sorts}}
```

Existing predicates:```
(*@\hlline{0.25}@*){{accumulated_predicates}}
```

Example:```
Sentence: Socrates is human.

Sorts:

- Person: An individual human being.

Predicates:

- IsHuman(Person): Indicates whether a person is human.

```


Analyze the request step by step, then respond with JSON in the following format
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}
\end{lstlisting}
\end{llmex}

==> figure/5_rule_formalizer.tex <==
\begin{llmex}{Prompt Template}
\begin{lstlisting}[style=llmtext]
You can perform the following actions.
Available Actions:
- write_dsl: Return exactly one DSL statement that conforms to the provided grammar for the given rule.
  Input Schema: {
  "type": "object",
  "properties": {
    "dsl": {
      "type": "string",
      "description": "A single DSL statement that ends with ';' and parses with the grammar."
    }
  },
  "required": [
    "dsl"
  ]
}


Write ONE DSL statement for the given natural-language rule, using the following Lark grammar.
Rules:
- The DSL must parse with this grammar.
- Do NOT invent predicate names or change arity; only use what appears in the grammar.
- Output exactly one statement and end it with ';'.
- If rule requires certain attributes from the target(provided in JSON format), use JSON path to access them.

Grammar:```
(*@\hlline{0.11}@*){{grammar}}
```

Natural-language rule:```
(*@\hlline{0.12}@*){{sentence}}
```


Associated Target:```
(*@\hlline{0.1}@*){{entity}}
```

Target Attributes in JSON format:```
(*@\hlline{0.2}@*){{entity_attributes}}
```

Analyze the request step by step, then respond with JSON in the following format
{
    "analysis": "Your analysis here",
    "actions": [
        {
            "name": "action_name",
            "input": {
                // action input according to the schema
            }
        }
    ]
}
\end{lstlisting}
\end{llmex}

==> figure/comparison_intro.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.8\linewidth]{image/compare_with_exisiting.png} 
    %\vspace{-0.2in}
    \mycaption{fig:compare_intro}{Comparison with existing solutions.}{}
\vspace{-0.1in}
\end{figure}

==> figure/fig-allavg.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=\linewidth]{image/allavg.png} 
    \vspace{-0.2in}
    \mycaption{fig:general}{Results with different LLMs.}{}
\vspace{-0.1in}
\end{figure}

==> figure/fig_ab.tex <==
\begin{figure*}[t]
\centering
\vspace{-0.1in}

\makebox[\textwidth]{%
\hfill
\includegraphics[width=0.24\textwidth]{image/ablation/legend.png}
\hfill
}
% Row 1: 3 graphics
\makebox[\textwidth]{%
\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/ablation/ERC20.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-erc20}{ERC20}
    {}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/ablation/ERC721.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-erc721}{ERC721}
    {}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/ablation/ERC1155.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-erc1155}{ERC1155}
    {}
    
\end{subfigure}  
\hfill
}


\vspace{0.02in}

% Row 2: 4 graphics
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/ablation/Rust1.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-rust1}{Rust-1}
    {}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/ablation/Rust2.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-rust2}{Rust-2}
    {}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/ablation/Java1.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-java1}{Java-1}
    {}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/ablation/Java2.png}
   \vspace{-0.1in}
  \mycaption{fig:ab-java2}{Java-2}
    {}
\end{subfigure}


\mycaption{fig:ablation}{Ablation on Doc2Spec components.}{}
\vspace{-0.1in}
\end{figure*}

==> figure/fig_general.tex <==
\begin{figure*}[t]
\centering
\vspace{-0.1in}

\makebox[\textwidth]{%
\hfill
\includegraphics[width=0.24\textwidth]{image/ablation/legend.png}
\hfill
}
% Row 1: 3 graphics
\makebox[\textwidth]{%
\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/general/ERC20.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-erc20}{ERC20}
    {}
\end{subfigure} 
\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/general/ERC721.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-erc721}{ERC721}
    {}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/general/ERC1155.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-erc1155}{ERC1155}
    {}
    
\end{subfigure}  
\hfill
}


\vspace{0.02in}

% Row 2: 4 graphics
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/general/Rust-1.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-rust1}{Rust-1}
    {}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/general/Rust-2.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-rust2}{Rust-2}
    {}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/general/Java-1.png}
  \vspace{-0.1in}
  \mycaption{fig:ab-java1}{Java-1}
    {}
\end{subfigure}\hfill
\begin{subfigure}[t]{0.24\textwidth}
  \centering
  \includegraphics[width=\linewidth]{image/general/Java-2.png}
   \vspace{-0.1in}
  \mycaption{fig:ab-java2}{Java-2}
    {}
\end{subfigure}


\mycaption{fig:general}{Doc2Spec with Different Models.}{}
\vspace{-0.1in}
\end{figure*}

==> image/erc20-example.tex <==
Transfers _value amount of tokens from address _from to address _to, and MUST fire the Transfer event.
The transferFrom method is used for a withdraw workflow, allowing contracts to transfer tokens on your behalf. This can be used for example to allow a contract to transfer tokens on your behalf and/or to charge fees in sub-currencies. (*@\hlline{0.12}@*)The (*@\hlline{0.48}@*)function SHOULD throw unless the _from account has (*@\hlline{0.72}@*)deliberately authorized the sender of the message (*@\hlline{0.28}@*)via some mechanism.
Note Transfers of 0 values MUST be treated as normal transfers and fire the Transfer event.
~function~ transferFrom(!address! _from, !address! _to, uint256 _value) public returns (bool success)

==> image/rust-example.tex <==
/// Deallocates the block of memory at the given `ptr` pointer with the given `layout`.
///
/// # Safety
///
/// The caller must ensure:
///
/// (*@\hlline{0.9}@*)* `ptr` is a block of memory currently allocated (*@\hlline{0.332}@*)via this allocator and,
///
/// * `layout` is the same layout that was used to allocate that block of
///   memory.
///
/// Otherwise undefined behavior can result.
#[stable(feature = "global_alloc", since = "1.28.0")]
unsafe fn dealloc(&self, ptr:*mut u8, layout:Layout);

==> sections/impact.tex <==
\section{Impact Statement}
This paper presents work whose goal is to advance the field of machine learning. There are many potential societal consequences of our work, none of which we feel must be specifically highlighted here.

==> tables/agent-feature.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Agent} & \textbf{CoT} & \textbf{Self-Refine}  & \textbf{One Shot} &\textbf{Self-Consistency \& Score} &  \textbf{Incremental Accumulation}  \\
\midrule
Entity Extractor   & \checkmark & \checkmark  &    \checkmark        &           & \checkmark  \\
Attribute Extractor   & \checkmark & \checkmark & \checkmark  &      &    \checkmark    \\
Rule Extractor        & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
Grammar Inferer     & \checkmark & \checkmark &  \checkmark         &  &  \checkmark    \\
Rule Formalizer       & \checkmark & \checkmark &   \checkmark        & \checkmark & \checkmark  \\
\bottomrule
\end{tabular}%
}
\mycaption{tab:agent-techniques}{Technique usage across agents. \checkmark indicates the technique is used.}{}

\end{table}

==> tables/agent-stats.tex <==
% Requires:
% \usepackage{booktabs, tabularx, makecell}
% (Optional) \usepackage{siunitx}  % nicer number alignment

\begin{table}[t]
\centering
\caption{Token usage and interaction turns per agent.}
\label{tab:agent-token-turns}
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabularx}{\linewidth}{l *{3}{>{\centering\arraybackslash}X}}
\toprule
\textbf{Agent} & \makecell{\textbf{\# In}\\\textbf{Tokens}} & \makecell{\textbf{\# Out}\\\textbf{Tokens}} & \makecell{\textbf{\#}\\\textbf{Turns}} \\
\midrule
Entity Extractor      & -- & -- & -- \\
Attribute Extractor     & -- & -- & -- \\
Rule Extractor     & -- & -- & -- \\
Predicate Inferer  & -- & -- & -- \\
Grammar Inferer   & -- & -- & -- \\
Rule Formalizer    & -- & -- & -- \\
\midrule
\textbf{Total}     & -- & -- & -- \\
\bottomrule
\end{tabularx}
\end{table}


==> tables/tbl-evaluation.tex <==
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{0.5pt}
\footnotesize
{
\mycaption{tab:results}
{Performance comparison with Precision(\%) and Recall(\%) reported. }
{
\textit{Numbers in brackets represent the Macro-F1 score(\%). Subscript indicates standard deviation(\%).}
}
\vspace{0.05in}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*} {} & \multicolumn{2}{c|}{\textbf{GPT} } & \multicolumn{2}{c|}{\textbf{Nemotron} } &  \multicolumn{2}{c|}{\textbf{Qwen3-32B} } &  \multicolumn{2}{c|}{\textbf{Qwen3-8B}} & \multicolumn{2}{c|}{\textbf{GPT w/o Grammar} }   \\
 \cline{2-11}
 & {\textbf{Precision}} & {\textbf{Recall}} & {\textbf{Precision}} &  {\textbf{Recall}}
 & {\textbf{Precision}} & {\textbf{Recall}} & {\textbf{Precision}} & {\textbf{Recall}}
 & {\textbf{Precision}} & {\textbf{Recall}} \\ \hline \hline


ERC20  & \pmstd{74.00}{4.35} & \pmstd{65.63}{9.38} &
  \pmstd{81.53}{0.49} & \pmstd{55.21}{1.80} &  
  \pmstd{78.70}{12.43} & \pmstd{44.79}{4.77} &  
  \pmstd{92.21}{7.23} & \pmstd{37.5}{6.25} & 
  \pmstd{46.39}{2.14} & \pmstd{45.83}{1.80} \\



ERC721  & \pmstd{53.68}{6.60}  & \pmstd{57.22}{3.85} &
\pmstd{68.65}{15.69} & \pmstd{41.11}{8.55} &
\pmstd{89.04}{8.06}  & \pmstd{37.22}{2.55} &
\pmstd{95.00}{0.00}  & \pmstd{31.67}{0.00} &
\pmstd{36.61}{0.80}  & \pmstd{53.89}{0.96} \\

ERC1155  &  \pmstd{78.60}{16.96} & \pmstd{86.67}{7.64} &
\pmstd{80.98}{5.21}  & \pmstd{64.17}{16.65} &
\pmstd{66.10}{34.05} & \pmstd{51.67}{1.44} &
\pmstd{100.00}{0.00} & \pmstd{34.17}{1.44} &
\pmstd{45.14}{3.74}  & \pmstd{84.17}{5.20} \\ \hline

Rust-1  & \pmstd{63.49}{14.42} & \pmstd{86.27}{13.58} &
\pmstd{83.57}{4.70}  & \pmstd{49.02}{3.40} &
\pmstd{87.88}{20.99} & \pmstd{47.06}{10.19} &
\pmstd{58.27}{37.63} & \pmstd{23.53}{0.00} &
\pmstd{31.63}{9.18}  & \pmstd{52.94}{5.88}  \\

Rust-2  &  \pmstd{46.34}{5.01}  & \pmstd{56.41}{5.88} &
\pmstd{28.00}{12.57} & \pmstd{26.92}{13.87} &
\pmstd{27.11}{16.84} & \pmstd{17.25}{3.89} &
\pmstd{33.95}{0.00} & \pmstd{21.79}{2.22} &
\pmstd{33.01}{0.56}  & \pmstd{44.21}{3.29} \\ \hline

Java-1  & \pmstd{90.19}{1.50}  & \pmstd{79.39}{11.87} &
\pmstd{83.07}{2.34}  & \pmstd{68.86}{2.01}  &
\pmstd{98.72}{2.22}  & \pmstd{33.77}{0.76}  &
\pmstd{100.00}{0.00} & \pmstd{14.94}{9.95}  &
\pmstd{54.72}{3.82}  & \pmstd{72.37}{3.95}   \\

Java-2  &  \pmstd{91.07}{5.87}  & \pmstd{89.31}{8.92}  &
\pmstd{69.98}{4.82}  & \pmstd{66.04}{6.80}  &
\pmstd{100.00}{0.00} & \pmstd{46.54}{2.88}  &
\pmstd{55.56}{50.92} & \pmstd{16.98}{23.19} &
\pmstd{61.51}{11.52} & \pmstd{87.42}{3.93}   \\ \hline 
\hline

Average  & \pmstd{71.05}{17.33} & \pmstd{74.41}{14.34} &
\pmstd{70.83}{19.87} & \pmstd{53.05}{15.21} &
\pmstd{78.22}{25.38} & \pmstd{39.76}{11.66} &
\pmstd{76.43}{25.37} & \pmstd{25.80}{8.74}  &
\pmstd{44.14}{11.23} & \pmstd{62.97}{18.09}   \\


% \bottomrule
\hline
\end{tabular}}
%\vspace{-0.15in}
\end{table*}


==> tables/tbl-extract-atoms.tex <==
\begin{table*}
\centering
\caption{Parameter Examples for \stepname{Extract Atoms}.}
\label{tab:segment}
\vspace{0.2em}
\footnotesize
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\setlength{\extrarowheight}{.75ex}
\begin{tabular}{|p{3.6cm}|p{6.7cm}|}
\hline
\textbf{Parameter} & \textbf{Example} \\
\hline
\hline
\textbf{RULE\_ID} & R0012 \\
\hline
\textbf{VERBATIM\_CLAUSE} & The function SHOULD throw unless the \_from account has deliberately authorized the sender of the message via some mechanism. \\
\hline
\textbf{TARGET\_DECLARATION} & function transferFrom(address \_from, address \_to, uint256 \_value) public returns (bool success) \\

\hline
\end{tabular}
\end{table*}
